Non-Extreme Individual Minima for Improved Pareto Front Sampling Efficiency and Decision-Making

In multi-objective optimization, the set of optimal trade-offs -- the Pareto front -- often contains regions that are extremely steep or flat. The Pareto optimal points in these regions are typically of limited interest for decision-making, as the marginal rate of substitution is extreme: a marginal improvement in one objective necessitates a significant deterioration in at least one other objective. These unfavorable trade-offs frequently occur near the individual minima, where single objectives attain their minimum values without considering the remaining criteria. To address this, we propose the concept of \emph{non-extreme individual minima} that relies on the notion of $L$-practical proper efficiency. These points can serve as a less sensitive replacement for \emph{standard} individual minima in subsequent related methods. Specifically, they allow for a more practical restriction of the Pareto front sampling within a refined utopia-nadir hyperbox, provide a meaningful basis for image space normalization, and can enhance decision-making techniques, such as knee-point methods, by focusing on regions with acceptable trade-offs. We provide a computationally efficient algorithm to determine these non-extreme individual minima by solving at most $2n_J$ standard weighted-sum scalarizations, where $n_J$ is the number of objectives. To ensure robustness across varying objective scales, the method incorporates an integrated image space normalization strategy. Numerical examples, specifically a convex academic case and a non-convex real-world application, demonstrate that the method successfully excludes practically irrelevant regions in the image space.

==> BuildFiles/header_hyperref.tex <==
\ifIFACClassFile
	\makeatletter
		\let\old@ssect\@ssect % Store how ifacconf defines \@ssect
	\makeatother	
	\usepackage{hyperref}
	\makeatletter
		\def\@ssect#1#2#3#4#5#6{%
				\NR@gettitle{#6}% Insert key \nameref title grab
			\old@ssect{#1}{#2}{#3}{#4}{#5}{#6}% Restore ifacconf's \@ssect
		}	
	\makeatother
\else
	\usepackage{hyperref}
\fi


	\hypersetup{
		draft=false,
		colorlinks=true,
		linkcolor = black,
		citecolor = black,
		urlcolor  = black,
		hypertexnames=false,
	}
	


	

